Prediction of Scene Plausibility

Understanding the 3D world from 2D images involves more than detection and segmentation of the objects within the scene. It also includes the interpretation of the structure and arrangement of the scene elements. Such understanding is often rooted in recognizing the physical world and its limitations, and in prior knowledge as to how similar typical scenes are arranged. In this research we pose a new challenge for neural network (or other) scene understanding algorithms - can they distinguish between plausible and implausible scenes? Plausibility can be defined both in terms of physical properties and in terms of functional and typical arrangements. Hence, we define plausibility as the probability of encountering a given scene in the real physical world. We build a dataset of synthetic images containing both plausible and implausible scenes, and test the success of various vision models in the task of recognizing and understanding plausibility.

==> future_work.tex <==
\section{Future Work}
We encourage the science community to continue and explore the problem of plausibility in images using our dataset and benchmark. Our code is available and can be used to generate additional data with no additional effort, and can easily be modified to create data of different types. In addition to finding a model that can detect the differences between plausible and implausible scenes, with some changes the data generation code can achieve a more diverse and complicated dataset: combining multiple implausibility categories in the same image, adding more texture for photo-realistic images and adding more scenes. 


==> intro-old.tex <==
\section{OLD Introduction}
When looking at a scene that contains multiple objects, one can easily decide if there is something improbable amongst those objects \cite{nightingale2017can}. Those improbabilities may appear in different forms in the same scene: a chair that floats in the air, a cup that is larger than a desk or shoes that are located on a bed. This contextual reasoning is a basic part of the human understanding of a scene \cite{chun1998contextual}. Furthermore, when an object is in an unreasonable context, we can usually recognize it. Although those tasks seem trivial for humans, when discussing machine learning algorithms we realize there are some challenges. In tasks such as scene classification, those obstacles affect the recognition of the entire scene; occurrences of objects in specific contexts allow the models to learn their class, and when the object appears out of that context, it results in an unrecognized object \cite{alcorn2019strike}, thus can give the scene an entirely different meaning \cite{laranjeira2019modeling}\cite{wu2015harvesting}. Many models focus on detecting and classifying scenes using local and global features, with any additional information supplied during the experiment. Usually the structure of the scene and the layout of the objects go unnoticed, unless used as a tool to serve this task \cite{hayat2016spatial}\cite{choi2012context}\cite{yao2012describing}. We claim that this is caused due to the lack of CNN based models ability to understand the layout of objects in a scene, and mostly perform detection tasks based on texture and shapes \cite{geirhos2018imagenet}. 

This context reasoning, or in other words, plausibility of a scene, is a subject that was learned through many different works in the field, although usually as a derivation of the tasks at hand, instead of the main focus of the study. 

When discussing the problem of implausibility in objects, there are several aspects to be taken into account \cite{bomatter2021pigs}:
1. Pose - impossible physical pose, 2. Location - impossible physical location, 3. Co-occurrences - unlikely object combinations, 4. Relative size - changes to the size of target objects relative to the other objects.


In addition to the benefits that may arise from detecting implausibility in scenes, classifying scenes’ plausibility is an important task for numerous reasons; many movies in the film industry are made using 3D models and then rendered. Those movies need to pass quality assurance, which is a human going through the entire movie checking for any incorrect rendering. Another example are GAN scene generators, some use input guidelines such as bounding boxes or sketches. The evaluation on those models are based on FID and IS \cite{salimans2016improved}\cite{heusel2017gans}, which are usually based on models that trained on single object images, allowing them to get a relatively high score even if the scene is implausible. 

When discussing the plausibility of a scene, we’re missing several basic building blocks to allow a proper research: (1) There is no score allowing to grade the plausibility of the object in the scene, hence preventing aggregation of those scores to a single scene score. (2) Lack of a large dataset to explore the problem. While there are many scene datasets available, most of them are in the wild, and none of them allow the transformation of the objects in an individual and controlled way. (3) No model is evaluated based on the capabilities of detecting implausible scenes. 


Our goals for this papers are:
\begin{itemize}
    \item Providing a formal definition to the problem of scene plausibility.
    \item Testing the current classification models when classifying implausibility of scenes
    \item Testing the current image evaluation models on implausible scenes
\end{itemize}



==> results.tex <==
\section{Results}

\begin{table}[h]
\begin{tabular}{|l|r|}
\hline
\textbf{Model} & \multicolumn{1}{c|}{\textbf{L1 Loss}} \\ \hline
ViT            & 0.289                                 \\ \hline
ORViT          & 0.289                                 \\ \hline
\end{tabular}
\end{table}
